The Two States of Star Forming Clouds

We examine the effects of self-gravity and magnetic fields on supersonic turbulence in isothermal molecular clouds with high resolution simulations and adaptive mesh refinement. These simulations use large root grids (512^3) to capture turbulence and four levels of refinement to capture high density, for an effective resolution of 8,196^3. Three Mach 9 simulations are performed, two super-Alfv\'enic and one trans-Alfv\'enic. We find that gravity splits the clouds into two populations, one low density turbulent state and one high density collapsing state. The low density state exhibits properties similar to non-self-gravitating in this regime, and we examine the effects of varied magnetic field strength on statistical properties: the density probability distribution function is approximately lognormal; velocity power spectral slopes decrease with field strength; alignment between velocity and magnetic field increases with field; the magnetic field probability distribution can be fit to a stretched exponential. The high density state is characterized by self-similar spheres; the density PDF is a power-law; collapse rate decreases with increasing mean field; density power spectra have positive slopes, P({\rho},k) \propto k; thermal-to-magnetic pressure ratios are unity for all simulations; dynamic-to-magnetic pressure ratios are larger than unity for all simulations; magnetic field distribution is a power-law. The high Alfv\'en Mach numbers in collapsing regions explain recent observations of magnetic influence decreasing with density. We also find that the high density state is found in filaments formed by converging flows, consistent with recent Herschel observations. Possible modifications to existing star formation theories are explored.

==> go <==
#!/bin/csh

set name = "ms"
set this_latex = latex
set this_latex = pdflatex
if( `grep  "^\\pdftrue" ms.tex |wc -l` == 1 ) set this_latex = pdflatex
if( `grep  "^\\pdffalse" ms.tex |wc -l` == 1 ) set this_latex = latex
if( -e /usr/bin/acroread ) then
 set run = "acroread"
else
 set run = "open"
endif    
rm -f *.log *.out *.aux *.dvi *~ *.bbl *.blg
rm -f *.ps  *.bak *.toc *.lof *.lot
rm $name.pdf

if( $1 == "c" ) then
    exit
endif

if( $1 == "o" ) then
    $this_latex $name
else
    
    ls -l
    
    $this_latex $name
    if( $status != 0 ) then
	echo "done borked sompin. Exiting."
	exit
    endif
    if ($1 != nb ) then
        bibtex $name
        $this_latex $name
        $this_latex $name
        mv ms.bbl derp.bbl
        #egrep -v "REVTEX41Control|????|apsrev41Control|^08. 1" derp.bbl > ms.bbl
        egrep -v "^ \?\?\?\?|^08. 1" derp.bbl > ms.bbl
        $this_latex $name
    endif
    if( $1 != "n" ) then
	if( -e $name.dvi ) then
	echo "convert to pdf"
	    dvips -Ppdf -t letter -o $name.ps $name.dvi
	    ps2pdf $name.ps $name.pdf

	    if( $status != 0 )then
		print "dvipdf borked.  That's *really* too bad."
		exit
	    endif
	endif
	if( $1 != "n" && ( -e $name.pdf ) ) $run $name.pdf &
    endif	    
endif
# the end

